SynEHRgy: Synthesizing Mixed-Type Structured Electronic Health Records using Decoder-Only Transformers

Generating synthetic Electronic Health Records (EHRs) offers significant potential for data augmentation, privacy-preserving data sharing, and improving machine learning model training. We propose a novel tokenization strategy tailored for structured EHR data, which encompasses diverse data types such as covariates, ICD codes, and irregularly sampled time series. Using a GPT-like decoder-only transformer model, we demonstrate the generation of high-quality synthetic EHRs. Our approach is evaluated using the MIMIC-III dataset, and we benchmark the fidelity, utility, and privacy of the generated data against state-of-the-art models.

==> tables/Excel2LaTeX/src/test/2x2.tex <==
% Table generated by Excel2LaTeX from sheet 'test'
\begin{tabular}{|r||r|}
\hline
1   & 2 \bigstrut\\
\hline
3   & 4 \bigstrut\\
\hline
\end{tabular}%


==> tables/Excel2LaTeX/src/test/empty-booktabs.tex <==
% Table generated by Excel2LaTeX from sheet 'test'
\begin{tabular}{r}

  \\
\end{tabular}%


==> tables/Excel2LaTeX/src/test/empty-convert.tex <==
% Table generated by Excel2LaTeX from sheet 'test'
\begin{tabular}{r}

  \\
\end{tabular}%


==> tables/Excel2LaTeX/src/test/empty-indent-3.tex <==
   % Table generated by Excel2LaTeX from sheet 'test'
   \begin{tabular}{r}
   
     \\
   \end{tabular}%


==> tables/Excel2LaTeX/src/test/empty-indent-5.tex <==
     % Table generated by Excel2LaTeX from sheet 'test'
     \begin{tabular}{r}
     
       \\
     \end{tabular}%


==> tables/Excel2LaTeX/src/test/empty-minwidth-1.tex <==
% Table generated by Excel2LaTeX from sheet 'test'
\begin{tabular}{r}
 \\
\end{tabular}%


==> tables/Excel2LaTeX/src/test/empty-table.tex <==
% Table generated by Excel2LaTeX from sheet 'test'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{r}
    
      \\
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> tables/Excel2LaTeX/src/test/empty.tex <==
% Table generated by Excel2LaTeX from sheet 'test'
\begin{tabular}{r}

  \\
\end{tabular}%


==> tables/Excel2LaTeX/src/test/fullrow.tex <==
% Table generated by Excel2LaTeX from sheet 'test'
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
    &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &     &  \\
\end{tabular}%


==> tables/Excel2LaTeX/src/test/multicol.tex <==
% Table generated by Excel2LaTeX from sheet 'test'
\begin{tabular}{rrrrr}
\multicolumn{2}{r}{1} &
  2 &
  \multicolumn{2}{r}{3}
  \\
\multicolumn{5}{r}{4}
  \\
5 &
  \multicolumn{3}{r}{6} &
  7
  \\
\end{tabular}%


==> tables/Excel2LaTeX/src/test/multirow.tex <==
% Table generated by Excel2LaTeX from sheet 'test'
\begin{tabular}{rrr}
\multirow{2}[0]{*}{1} &
  \multirow{5}[0]{*}{4} &
  5
  \\
 &
   &
  \multirow{3}[0]{*}{6}
  \\
2 &
   &
  
  \\
\multirow{2}[0]{*}{3} &
   &
  
  \\
 &
   &
  7
  \\
\end{tabular}%


==> tables/Excel2LaTeX/src/test/multirowcol.tex <==
% Table generated by Excel2LaTeX from sheet 'test'
\begin{tabular}{rrrrrr}
\multicolumn{2}{r}{\multirow{2}[0]{*}{1}} &
  2 &
  3 &
  4 &
  5
  \\
\multicolumn{2}{r}{} &
  6 &
  7 &
  8 &
  9
  \\
0 &
  1 &
  2 &
  3 &
  4 &
  5
  \\
6 &
  7 &
  8 &
  \multicolumn{3}{r}{\multirow{3}[0]{*}{9}}
  \\
0 &
  1 &
  2 &
  \multicolumn{3}{r}{}
  \\
3 &
  4 &
  5 &
  \multicolumn{3}{r}{}
  \\
\end{tabular}%


==> tables/Excel2LaTeX/src/test/special-convert.tex <==
% Table generated by Excel2LaTeX from sheet 'test'
\begin{tabular}{l}
\$\textbackslash{}delta\_1\^2+\textbackslash{}delta\_2\^2 = \textbackslash{}gamma\^2\$\newline{}is \textbackslash{}textbf{true} \\
\end{tabular}%


==> tables/Excel2LaTeX/src/test/special.tex <==
% Table generated by Excel2LaTeX from sheet 'test'
\begin{tabular}{l}
$\delta_1^2+\delta_2^2 = \gamma^2$\newline{}is \textbf{true} \\
\end{tabular}%

